Exploring LLM Cryptocurrency Trading Through Fact-Subjectivity Aware Reasoning

While many studies show that more advanced LLMs excel in tasks such as mathematics and coding, we observe that in cryptocurrency trading, stronger LLMs sometimes underperform compared to weaker ones. To investigate this counterintuitive phenomenon, we examine how LLMs reason when making trading decisions. Our findings reveal that (1) stronger LLMs show a preference for factual information over subjectivity; (2) separating the reasoning process into factual and subjective components leads to higher profits. Building on these insights, we propose a multi-agent framework, FS-ReasoningAgent, which enables LLMs to recognize and learn from both factual and subjective reasoning. Extensive experiments demonstrate that this fine-grained reasoning approach enhances LLM trading performance in cryptocurrency markets, yielding profit improvements of 7\% in BTC, 2\% in ETH, and 10\% in SOL. Additionally, an ablation study reveals that relying on subjective news generates higher returns in bull markets, while focusing on factual information yields better results in bear markets. Code is available at https://github.com/Persdre/FS-ReasoningAgent.

==> sec-analysis.tex <==
\section{Demystifying LLM Reasoning in Trading}
% In our preliminary experiments, the LLMs are given market statistics, including 7-day opening and closing prices, MACD, and related news. Advanced commonly used LLMs including GPT-3.5-turbo, GPT-4, GPT-4o and GPT-4o-mini. Normally, the reasoning ability of them is xxxxxxxxxxxxxx, which is evaluated based on the tasks xxxxxxxxxxxxx.

% Table~\ref{} shows that for ETH, stronger LLMs do not have higher returns than weaker LLMs as expected. In addition, less favorable risk adjusted performance (sharpe ratio) of stronger LLMs is observed. Similar trends are observed in the results for BTC and SOL (provided in Appendix xx). 


In this section, we analyze this counterintuitive phenomenon and partially interpret why stronger LLMs with advanced reasoning ability fail to outperform weaker ones in trading.

% Normally, stronger LLMs show better long-context understanding ability \cite{}.

\textbf{Failing to capture important information.} In the context of financial markets, the news plays a pivotal role in influencing the prices of various assets \cite{rubinstein2001rational, meltzer2002rational}. Due to the huge message length like news, the input messages are actually very long contexts for LLMs. Stronger LLMs normally have better in-context learning abilities. However, due to their current limitations of the long-context understanding problems \cite{},  it is difficult for LLMs to simultaneously understand all news and make precise trading decisions. Thus, even for stronger LLMs, some important information that hide in the news sea cannot be well captured like the needle-in-stack experiments ~\cite{}.

Given this backdrop, we suppose that LLMs have different understandings of the news contents and make different trading decisions. Based on this, we introduce two agents to extract the news into factual and subjective parts, which are the two most influential factors on prices ~\cite{}. Figure~\ref{fig:reasoning} shows how different LLMs extract factual news and subjective news. With this xxxxxxxxxxxx.
\textcolor{red}{we may need an extra simple additional experiment here....}



\textbf{Failing to adjust trading strategies.} LLMs are basically trained with different data sets. Thus, different preferences and prior knowledge about trading are encoded in their weights. However, the market is dynamic and completely different from the training data in LLMs. The stale trading strategies may not be continuously used in the new market. Thus, we require the LLM to make trading decisions based on statistical prices and the demystified news summarized by the factual and subjective agents. The comparison reasoning processes in \autoref{fig:reasoning} shows that different LLMs finnaly make different trading decisions, thus resulting different returns. However, there trading agents do not have any feedbacks to allow them to adjust their trading strategies according to the market environments. This results in that LLMs excessively depend on their past experience (training datasets) to make the trading decisions.


% the strong LLMs may misunderstand 
% And different LLMs have different prior knowledge and preferences on the trading strategies. 



















